Reward-Directed Conditional Diffusion: Provable Distribution Estimation and Reward Improvement

We explore the methodology and theory of reward-directed generation via conditional diffusion models. Directed generation aims to generate samples with desired properties as measured by a reward function, which has broad applications in generative AI, reinforcement learning, and computational biology. We consider the common learning scenario where the data set consists of unlabeled data along with a smaller set of data with noisy reward labels. Our approach leverages a learned reward function on the smaller data set as a pseudolabeler. From a theoretical standpoint, we show that this directed generator can effectively learn and sample from the reward-conditioned data distribution. Additionally, our model is capable of recovering the latent subspace representation of data. Moreover, we establish that the model generates a new population that moves closer to a user-specified target reward value, where the optimality gap aligns with the off-policy bandit regret in the feature subspace. The improvement in rewards obtained is influenced by the interplay between the strength of the reward signal, the distribution shift, and the cost of off-support extrapolation. We provide empirical results to validate our theory and highlight the relationship between the strength of extrapolation and the quality of generated samples.

==> arxiv/section/tem_proofs_non.tex <==
\section{Moving from maintext_nonparametric}
\paragraph{Score Matching Error in $s_{\hat w}$} 
\begin{align*}
\frac{1}{T - t_0} \int_{t_0}^T \EE_{x, \hat f} \norm{\nabla_x \log p_t(x, \hat f) - s_{\hat w}(x, \hat f, t)}_2^2 \diff t \leq \epsilon^2_{diff} (N_d).
\end{align*}
Suppose $\nabla_x \log p_t(x, \hat f)$ is within a parametric family $\cS$ and the $s_{w^*} (x, \hat f, t) = \nabla_x \log p_t(x, \hat f)$, then
\begin{equation*}
    \epsilon_{diff} (N_d) = \frac{|\cS|}{\sqrt{N_d}}.
\end{equation*}

\begin{comment}
The score function can be computed as
\begin{align*}
\nabla \log p_t(\xb) = \underbrace{- A \Sigma_t^{-1} A^\top \xb}_{\sbb_\parallel}\underbrace{  - \frac{1}{h(t)} (I_D - AA^\top)\xb}_{\sbb_{\perp}},
\end{align*}
where $\Sigma_t = \diag(\dots,  \alpha^2(t) \lambda_k^2 + h(t) , \dots)$.

One can verify that $\sbb_{\parallel}$ now is linear in $\xb$, whereas $\sbb_{\perp}$ blows up when $t$ approaches $0$. Moreover, only the on-support score $\sbb_{\parallel}$ carries the covariance information of the latent distribution and will guide the distribution recovery.

A closer evaluation further reveals $\pscore$ is Lipschitz continuous, i.e.,
\begin{align*}
\norm{\pscore(\zb_1, t) - \pscore(\zb_2, t)}_{2} \leq \max\{\lambda_d^{-2}, 1 \}\norm{\zb_1 - \zb_2}_2
\end{align*}
for any $t \in [0, T]$ and $\zb_1, \zb_2$, and
\begin{align*}
\norm{\pscore(\zb, t_1) - \pscore(\zb, t_2)}_{2} \leq \max\{\lambda_d^{-2}, 1\} \norm{\zb}_2 |t_1 - t_2|.
\end{align*}
for any $\zb$ and $t_1, t_2 \in [0, T]$. Such properties are essential to develop score approximation and estimation results.
\end{comment}

\paragraph{Regression Error in $\hat f$}
Regression on $\cD_{label}$ leads to 
\begin{align}
\label{equ:rgs_error}
\EE \left[\norm{f^{\star} - \hat{f}}_{L^2(P_{x})}^2\right] \leq \epsilon_{reg} ^2 (N_{r}).
\end{align}

\paragraph{Distribution Shift}
Divergence $\chi^2_{\cG} (p,q)$ is defined as
\begin{align*}
\chi^2_{\cG} (p,q) = \sup_{g \in \cG} \frac{\EE_{p}[g]}{\EE_{q}[g]}.
\end{align*}

\begin{lemma}
\label{lmm:imprv_per_step}
Generating $x$ from $\hat{P}(x | \hat f(x) = a)$ with inputs $a \sim q$ has a guarantee of $f^{\star}(x)$ that
\begin{align}
    \nonumber \EE_{a \sim q} \EE_{x \sim \hat{P}(x | \hat f(x) = a)} [f^{\star}(x)] \geq &\EE_{a \sim q} [a] - 
    2 \norm{\hat f}_\infty \cdot \sqrt{\chi^2_{\cR_{\cS}} (P_{x \hat f}, P_{x|\hat f} \times q)} \cdot \epsilon_{diff} (N_{d})\\
    \label{equ:improvement}&- \sqrt{\chi^2_{\cR_{\cF}} (\hat{p}_q,p)}  \cdot \epsilon_{reg}(N_r).
\end{align}
where $p(x)$ is the density of the marginal distribution of $x$ in $\cD_{label}$, $\hat p_q (x):= \int q(a)\hat{p}(x | \hat f = a)\diff a$ denotes the generated density with input $a \sim q$. We shall take 
\begin{align*}
    \cR_{\cS}&:= \left\{\norm{\nabla_x \log p_t(x, \hat f) - s_w(x, \hat f, t)}_2^2 : s_w \in \cS \right\},\\
    \cR_{\cF}&:= \{|f^* - f|^2: f \in \cF\},
\end{align*}
$\cF$ is the function class to approximate $f^*$.
\end{lemma}

We consider an i.i.d. logged data set consisting of $n$ pairs $(x_i, y_i)$ for $i = 1, \dots, n$. Here $x \in \RR^d$ is the feature, and $y \in \RR$ is a noisy response generated by $y = f^{\star}(x) + \xi$, where $f^{\star}$ is some Lipschitz function and independent noise $\xi$ is Gaussian distributed as ${\sf N}(0, \sigma^2 I)$. We denote the joint sampling distribution on $(x, y)$ as $P_{xy}$. Also we use notation $P_t$ to denote the the joint distribution of $(x,y)$ at time $t$ where $x$ is diffused with Gaussian noise. $p_t(x,y)$ is the corresponding density.
\begin{assumption}
We assume $P_{xy}$ has a density function $p_{xy}$, such that there exists constants $B, C_1, C_2$ verifying $p_{xy}(x, y) \leq (2\pi)^{-(d+1)/2} C_1 \exp\left(-C_2 \norm{x}_2^2 / 2\right)$ whenever $\norm{x}_2 > B$.
\end{assumption}

\begin{assumption}
The score function $\nabla_x \log p_t(x, y)$ of $P_{xy}$ is Lipschitz for any $t \in [t_0, T]$, i.e., there exists a constant $L$, such that for any $x, y$ and $x^{\prime}, y^{\prime}$, it holds
\begin{align*}
\norm{\nabla_x \log p_t(x, y) - \nabla_x \log p_t(x^{\prime}, y^{\prime})}_2 \leq L \norm{x - x^{\prime}}_2 + L\norm{y - y^{\prime}}_2.
\end{align*}
\end{assumption}

\paragraph{Score matching} 
\begin{comment}
We diffuse on $x$ and $y$ jointly. A conceptual loss for score matching is
\begin{align*}
\min_{\theta} \int_{0}^T \EE_{x, y} \left[\norm{\nabla_x \log p_t(x, y) - s_\theta(x, y, t)}_2^2\right] \diff t.
\end{align*}
Note that we have the identity $\nabla_x \log p_t(x | y) = \nabla_x \log p_t(x, y)$. Therefore, the objective function above can also be viewed as estimating the conditional score. To allow practical implementation, we resort to the following equivalent objective,
\begin{align*}
\min_{\theta} \int_{0}^T \EE_{x, y} \left[\EE_{x^{\prime} \sim {\sf N}(\alpha(t)x, h(t)I)}\left[\norm{\nabla_x \log \phi_t(x^{\prime} | x) - s_\theta(x^{\prime}, y, t)}_2^2\right]\right] \diff t,
\end{align*}
whose equivalence is established in Lemma \ref{lemma:obj_equal}.
The remaining analysis follows \url{https://arxiv.org/abs/2302.07194}, with $A = I$.
\end{comment}
We diffuse on $x$ and maintain $y$.  It applies no matter $y$ is a deterministic function of $x$ (i.e. the case where $y = \hat f(x)$) or $y$ is a noisy reward feedback of $f^{\star}(x)$ (i.e. $y = f^{\star}(x) + \xi$) that for $\forall t \not = 0$
\begin{equation}
\label{equ:cdt_score}
    \nabla_x \log p_t(x \mid y) = \nabla_x \log p_t(x , y).
\end{equation}
And all densities in (\ref{equ:cdt_score}) are well-defined. Thus, a conceptual loss of score matching for sampling conditionally is
\begin{align*}
\min_{\theta} \int_{t_0}^T \EE_{x, y} \left[\norm{\nabla_x \log p_t(x, y) - s_\theta(x, y, t)}_2^2\right] \diff t.
\end{align*}

The remaining analysis follows \url{https://arxiv.org/abs/2302.07194}, with $A = I$.

We configure the ReLU network $s_\theta(x, y, t): R^{d+2} \to R^{d}$ by hyperparameters. Specifically, $s_\theta(x, y, t) \in \mathcal{S}_{\mathrm{NN}}\left(L, M, J, K, \kappa, \gamma, \gamma_t\right)$ with
$$
\begin{aligned}
\mathcal{S}_{\mathrm{NN}}\left(L, M, J, K, \kappa, \gamma, \gamma_t\right)=\{ & s_{\theta}(\mathbf{z}, t)=W_L \sigma\left(\ldots \sigma\left(W_1\left[\mathbf{z}^{\top}, t\right]^{\top}+\mathbf{b}_1\right) \ldots\right)+\mathbf{b}_L: \\
& \mathbf{z} = (x,y) \in R^{d+1}, \\
& \text { network width bounded by } M, \sup _{\mathbf{z}, t}\|s_{\theta}(\mathbf{z}, t)\|_2 \leq K, \\
& \max \left\{\left\|\mathbf{b}_i\right\|_{\infty},\left\|W_i\right\|_{\infty}\right\} \leq \kappa \text { for } i=1, \ldots, L, \\
& \sum_{i=1}^L\left(\left\|W_i\right\|_0+\left\|\mathbf{b}_i\right\|_0\right) \leq J, \\
& \left\|s_{\theta}\left(\mathbf{z}_1, t\right)-s_{\theta}\left(\mathbf{z}_2, t\right)\right\|_2 \leq \gamma\left\|\mathbf{z}_1-\mathbf{z}_2\right\|_2 \text { for any } t \in[0, T], \\
& \left.\left\|s_{\theta}\left(\mathbf{z}, t_1\right)-s_{\theta}\left(\mathbf{z}, t_2\right)\right\|_2 \leq \gamma_t\left|t_1-t_2\right| \text { for any } \mathbf{z}\right\},
\end{aligned}
$$
where the network width refers to the maximum dimensions of the weight matrices, $\sigma$ is the ReLU activation, and $\|\cdot\|_{\infty}$ and $\|\cdot\|_0$ denote the maximum magnitude of entries and the number of nonzero entries, respectively. In the sequel, we write $\mathcal{S}_{\mathrm{NN}}\left(L, M, J, K, \kappa, \gamma, \gamma_t\right)$ to reflect the configuration of $\mathrm{f}_\theta$.

\begin{theorem}
\label{thm:NN}
Given an approximation error $\epsilon>0$, we choose $\mathcal{S}_{\mathrm{NN}}$ with
$$
\begin{aligned}
L & =\mathcal{O}\left(\log \frac{1}{\epsilon}+d\right), K=\mathcal{O}\left(2 d^2 \log \left(\frac{d}{t_0 \epsilon}\right)\right) \\
M & =\mathcal{O}\left((1+\beta)^d T \tau d^{d / 2+1} \epsilon^{-(d+1)} \log ^{d / 2}\left(\frac{d}{t_0 \epsilon}\right)\right) \\
J & =\mathcal{O}\left((1+\beta)^d T \tau d^{d / 2+1} \epsilon^{-(d+1)} \log ^{d / 2}\left(\frac{d}{t_0 \epsilon}\right)\left(\log \frac{1}{\epsilon}+d\right)\right) \\
\kappa & =\mathcal{O}\left(\max \left\{2(1+\beta) \sqrt{d \log \left(\frac{d}{t_0 \epsilon}\right)}, T \tau\right\}\right) \\
\gamma & =10 d(1+\beta), \gamma_t=10 \tau
\end{aligned}
$$
where $\tau=\sup _{t \in\left[t_0, T\right]} \sup _{\|\mathbf{z}\|_{\infty}} \leq \sqrt{d \log \frac{d}{t_0 \epsilon}}\left\|\frac{\partial}{\partial t}\left[h(t) \mathbf{s}_{\|}(\mathbf{z}, t)\right]\right\|_2$. Then for any data distribution $P_{x,y}$ satisfying Assumptions \ref{asmp:tail} and \ref{asmp:lipschitz}, there exists an $\overline{\mathbf{s}}_{\boldsymbol{\theta}} \in \mathcal{S}_{\mathrm{NN}}$ such that for any $t \in\left[t_0, T\right]$, we have
$$
\left\|\overline{\mathbf{s}}_{\boldsymbol{\theta}}(x,y, t)-\nabla \log p_t(x,y)\right\|_{L^2\left(P_t\right)} \leq \frac{\sqrt{d}+1}{h(t)} \epsilon .
$$
\end{theorem}

\begin{theorem}
Suppose Assumptions \ref{asmp:tail} and \ref{asmp:lipschitz} hold. We choose $\mathcal{S}_{\mathrm{NN}}$ as in Theorem \ref{thm:NN} with $\epsilon=n^{-\frac{1-\delta(n)}{d+5}}$ for $\delta(n)=\frac{d \log \log n}{\log n}$. Then with probability $1-\frac{1}{n}$, it holds
$$
\frac{1}{T-t_0} \int_{t_0}^T\left\|\widehat{\mathbf{s}}_{ \boldsymbol{\theta}}(x,y, t)-\nabla \log p_t(x,y)\right\|_{L^2\left(P_t\right)}^2 \mathrm{~d} t=\widetilde{\mathcal{O}}\left(\frac{1}{t_0}\left(n^{-\frac{2-2 \delta(n)}{d+5}}+D n^{-\frac{d+3}{d+5}}\right) \log ^3 n\right)
$$
where $\widetilde{\mathcal{O}}$ hides factors depending on $\beta, \log D, d, \log t_0$ and $\tau$ defined in Theorem \ref{thm:NN} .
\end{theorem}

\paragraph{Distribution shift}
Analysis above yields
\begin{align*}
\frac{1}{T - t_0} \int_{t_0}^T \EE_{x, y} \norm{\nabla_x \log p_t(x, y) - s_\theta(x, y, t)}_2^2 \diff t \leq \epsilon_{diff} (N)
\end{align*}
for some $\epsilon$ dependent on sample size $N$ and other hyperparameters.

We translate it to an upper bound under the conditional distribution $P(x | y) \times q_y$, for $q_y$ being a prior distribution on $y$. In particular, we have
\begin{align*}
& \int_{t_0}^T \EE_{y \sim q_y} \EE_{x | y} \norm{\nabla_x \log p_t(x, y) - s_\theta(x, y, t)}_2^2 \diff t \\ & \quad \leq \chi^2_{\cG}(P_{xy}, P_{x | y} \times q_y) \int_{t_0}^T \EE_{x, y} \norm{\nabla_x \log p_t(x, y) - s_\theta(x, y, t)}_2^2 \diff t,
\end{align*}
where divergence $\chi^2_{\cF}$ is defined as
\begin{align*}
\chi^2_{\cF} (P_{xy}, P_{x|y} \times q_y) = \sup_{g \in \cG} \frac{\EE_{P_{xy}}[g]}{\EE_{P_{x|y} \times q_y}[g]}.
\end{align*}
We shall take $\cG$ as $\left\{\norm{\nabla_x \log p_t(x, y) - s_\theta(x, y, t)}_2^2 : s_\theta \in \cS \right\}$.

